Simulationsverfahren fuer Brown-Resnick-Prozesse (Simulation Techniques for Brown-Resnick Processes)

Generalized Brown-Resnick processes form a flexible class of stationary max-stable processes based on Gaussian random fields. With regard to applications fast and accurate simulation of these processes is an important issue. In fact, Brown-Resnick processes that are generated by a dissipative flow do not allow for good finite approximations using the definition of the processes. On large intervals we get either huge approximation errors or very long operating times. Looking for solutions of this problem, we give different representations of the generalized Brown-Resnick processes - including random shifting and a mixed moving maxima representation - and derive various kinds of finite approximations that can be used for simulation purposes. Furthermore, error bounds are calculated in the case of the original process by Brown and Resnick (1977).

==> Anhang.tex <==
\chapter{Code der zur Simulation verwendeten Funktionen}

Zur Simulation von Brown-Resnick-Prozessen auf $\R$ werden die \texttt{R-Funktionen} \texttt{meth0, meth1, meth2, meth3, meth4} und die entsprechenden \texttt{C}-Funktionen sowie zur Sch"atzung des Parameters $\lambda^*$ die \texttt{R}-Funktion \texttt{findlambda} verwendet. Der Code wird hier bereitgestellt. Auf den Code der intern verwendeten Funktionen zur Simulation (intrinsisch) station"arer Zufallsfelder aus dem \texttt{R}-Package \texttt{RandomFields} (Version 2.0.14) von Martin Schlather soll an dieser Stelle nicht n"aher eingegangen werden.
\medskip

Die \texttt{R}-Funktionen sind in der Datei \texttt{methods.R} codiert:
\lstset{ 
language=R,                % choose the language of the code
basicstyle=\scriptsize,       % the size of the fonts that are used for the code
numbers=left,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=2,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,	                % adds a frame around the code
tabsize=2,	                % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
deletekeywords={step, model, lower, upper},
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}
\lstinputlisting{RFBR/R/methods.R}


Als Header-Datei f"ur die integrierten \texttt{C}-Funktionen verwenden wir \texttt{RFBR.h}:
\lstset{ %
language=C,                % choose the language of the code
basicstyle=\scriptsize,       % the size of the fonts that are used for the code
numbers=left,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=2,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,	                % adds a frame around the code
tabsize=2,	                % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
}

\lstinputlisting{RFBR/src/RFBR.h}
\newpage

Die \texttt{C}-Funktionen selbst sind schlie"slich in der Datei \texttt{methods.cc} codiert:
\lstset{ %
language=C,                % choose the language of the code
basicstyle=\scriptsize,       % the size of the fonts that are used for the code
numbers=left,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=2,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,	                % adds a frame around the code
tabsize=2,	                % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
}

\lstinputlisting{RFBR/src/methods.cc}


Der bestehende Code aus \texttt{RandomFields} ist im Vergleich zu Version 2.0.14 nur insofern ver"andert, dass bei allen Aufrufen von \texttt{C}-Funktionen aus \texttt{R} (mittels \texttt{.C} oder \texttt{.Call}) die Option \texttt{PACKAGE="RandomFields"} durch \texttt{PACKAGE="RFBR"} ersetzt ist.



\chapter{Dokumentation der zur Simulation verwendeten \texttt{R}-Funktionen}

Zur Verwendung der Funktionen seien die folgenden Artikel aus der Package-Dokumentation empfohlen.

\input{meth0}
\bigskip
\input{meth1}
\bigskip
\input{meth2}
\bigskip
\input{meth3}
\bigskip
\input{meth4}

\chapter{\texttt{R}-Skript und Ergebnisse der Simulationsstudie}

Im Folgenden werden die detaillierten Ergebnisse der Simulationsstudie, die in Kapitel 4 der Arbeit ausgewertet wird, vorgestellt.

Das $\texttt{R}$-Skript, das zu diesen Ergebnissen f"uhrt, sei hier exemplarisch f"ur $\alpha = 0.1$ angegeben:

\lstset{ %
language=R,                % choose the language of the code
basicstyle=\scriptsize,       % the size of the fonts that are used for the code
numbers=left,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=2,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,	                % adds a frame around the code
tabsize=2,	                % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
deletekeywords={step, model, lower, upper},
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}


\lstinputlisting{RFBR/tests/BRsim.R}


Der Output besteht aus Informationen zu den Methoden und den gew"ahlten Parametern und daneben den Kennziffern \texttt{dev(a)}, \texttt{dev(0)}, \texttt{dev(b)} und \texttt{DEV}.

Dabei handelt es sich um die maximale Abweichung der empirischen Randverteilungsfunktion von der Standard-Gumbel"=Verteilungsfunktion an den Stellen \texttt{a}, 0 und \texttt{b}, also in der Mitte und an den R"andern des Intervalls, sowie um das arithmetische Mittel aus $\texttt{dev(a)}$ und $\texttt{dev(b)}$. Letztere Gr"o"se ist -- wie in Kapitel 4 beschrieben -- die entscheidende Kennzahl zum Vergleich der Methoden.
\bigskip

Hier die Ergebnisse f"ur $\alpha=0.1$:

\lstinputlisting{printres/res01.txt}

\medskip

f"ur $\alpha = 0.5$:

\lstinputlisting{printres/res05.txt}

\newpage

f"ur $\alpha = 1$:

\lstinputlisting{printres/res10.txt}

\medskip

f"ur $\alpha = 1.5$:

\lstinputlisting{printres/res15.txt}

\medskip

und schlie"slich f"ur $\alpha = 1.9$:

\lstinputlisting{printres/res19.txt}

